Uncovering In-DRAM RowHammer Protection Mechanisms: A New Methodology, Custom RowHammer Patterns, and Implications

The RowHammer vulnerability in DRAM is a critical threat to system security. To protect against RowHammer, vendors commit to security-through-obscurity: modern DRAM chips rely on undocumented, proprietary, on-die mitigations, commonly known as Target Row Refresh (TRR). At a high level, TRR detects and refreshes potential RowHammer-victim rows, but its exact implementations are not openly disclosed. Security guarantees of TRR mechanisms cannot be easily studied due to their proprietary nature. To assess the security guarantees of recent DRAM chips, we present Uncovering TRR (U-TRR), an experimental methodology to analyze in-DRAM TRR implementations. U-TRR is based on the new observation that data retention failures in DRAM enable a side channel that leaks information on how TRR refreshes potential victim rows. U-TRR allows us to (i) understand how logical DRAM rows are laid out physically in silicon; (ii) study undocumented on-die TRR mechanisms; and (iii) combine (i) and (ii) to evaluate the RowHammer security guarantees of modern DRAM chips. We show how U-TRR allows us to craft RowHammer access patterns that successfully circumvent the TRR mechanisms employed in 45 DRAM modules of the three major DRAM vendors. We find that the DRAM modules we analyze are vulnerable to RowHammer, having bit flips in up to 99.9% of all DRAM rows. We make U-TRR source code openly and freely available at [106].

==> Makefile <==
PAPER=main
PDF_NAME=utrr_arxiv_draft

default: paper

paper:
	pdflatex --jobname=$(PDF_NAME) $(PAPER).tex </dev/null
	bibtex $(PDF_NAME)
	pdflatex --jobname=$(PDF_NAME) $(PAPER).tex </dev/null >/dev/null
	pdflatex --jobname=$(PDF_NAME) $(PAPER).tex </dev/null >/dev/null
	pdflatex --jobname=$(PDF_NAME) $(PAPER).tex </dev/null

tidy:
	rm -f $(PAPER).aux $(PAPER).bbl $(PAPER).blg $(PAPER).brf $(PAPER).btx $(PAPER).log $(PAPER).out
	rm -f $(PDF_NAME).aux $(PDF_NAME).bbl $(PDF_NAME).blg $(PDF_NAME).brf $(PDF_NAME).btx $(PDF_NAME).log $(PDF_NAME).out

clean: tidy
	rm -f $(PAPER).pdf $(PDF_NAME).pdf

# PDF = main.pdf

# all: ${PDF}

# %.pdf: %.tex acmart.cls ACM-Reference-Format.bst
# 	pdflatex $<
# 	- bibtex $*
# 	pdflatex $<
# 	pdflatex $<
# 	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
# 	do pdflatex $<; done

# clean:
# 	$(RM) *.log *.aux \
# 	*.cfg *.glo *.idx *.toc \
# 	*.ilg *.ind *.out *.lof \
# 	*.lot *.bbl *.blg *.gls *.cut *.hd \
# 	*.dvi *.ps *.thm *.tgz *.gz *.zip *.rpi \
#   $(PDF) *-converted-to.pdf

